PaReNTT: Low-Latency Parallel Residue Number System and NTT-Based Long Polynomial Modular Multiplication for Homomorphic Encryption

High-speed long polynomial multiplication is important for applications in homomorphic encryption (HE) and lattice-based cryptosystems. This paper addresses low-latency hardware architectures for long polynomial modular multiplication using the number-theoretic transform (NTT) and inverse NTT (iNTT). Chinese remainder theorem (CRT) is used to decompose the modulus into multiple smaller moduli. Our proposed architecture, namely PaReNTT, makes four novel contributions. First, parallel NTT and iNTT architectures are proposed to reduce the number of clock cycles to process the polynomials. This can enable real-time processing for HE applications, as the number of clock cycles to process the polynomial is inversely proportional to the level of parallelism. Second, the proposed architecture eliminates the need for permuting the NTT outputs before their product is input to the iNTT. This reduces latency by n/4 clock cycles, where n is the length of the polynomial, and reduces buffer requirement by one delay-switch-delay circuit of size n. Third, an approach to select special moduli is presented where the moduli can be expressed in terms of a few signed power-of-two terms. Fourth, novel architectures for pre-processing for computing residual polynomials using the CRT and post-processing for combining the residual polynomials are proposed. These architectures significantly reduce the area consumption of the pre-processing and post-processing steps. The proposed long modular polynomial multiplications are ideal for applications that require low latency and high sample rate as these feed-forward architectures can be pipelined at arbitrary levels.

==> response.tex <==
\onecolumn
\pagenumbering{arabic} 

\section*{Response to the reviewers:  T-IFS-15464-2022}
% \noindent \textbf{Manuscript ID:} TC-2021-10-0542\\
% \textbf{Title:} Low-Latency VLSI Architectures for Modular Polynomial Multiplication via Fast Filtering and Applications to Lattice-Based Cryptography\\
% \textbf{Authors:} Weihang Tan, Antian Wang, Xinmiao Zhang, Yingjie Lao, and Keshab K. Parhi.\\
% \textbf{To:} Editor in Chief, IEEE Transactions on Computers\\
% % General intro text goes here
% We sincerely appreciate the Associate Editor and reviewers' constructive comments for helping us improve our work. We are grateful for the comments of all the reviewers. The manuscript is revised carefully and point-by-point answers to the comments are provided below.
The authors appreciate the numerous constructive comments from the two reviewers. All comments have been incorporated in the revised version. A list of changes is summarized below.
\begin{itemize}
  
\item The description of the NTT and iNTT algorithms is moved to the Supplementary Information. Instead, the flow graphs for the low-complexity negative wrapped convolution NTT and iNTT structures are now shown in the paper.
\item The expansion of the feasible moduli set is explained better. New results for the expansion of the number of feasible prime factors are now presented.
\item A new algorithm is presented for reducing complexity of the residual computation unit of the CRT implementation. This algorithm, based on decomposition, reduces the hardware complexity when the number of moduli is large.
\item New results for area and time for the stand-alone preprocessing and postprocessing parts of the CRT are now presented. Pipelinining tradeoffs of these circuits are also described.
\item Several new experimental results are presented. Power consumption of the final circuit is also included.

\end{itemize}

\reviewersection
Comments:
In this paper, the authors propose parallel NTT architectures for real-time holomorphic encryption applications. They have low-latency hardware architectures for long polynomial multiplication. They also provide some architectures for Chinese Remainder Theorem and the residual polynomials. According to the experimental results, the proposed idea reduces the area-block processing. The idea is interesting. I think it deserves to be known. However, I am not sure that this is the venue for this topic. In my opinion Journal of Cryptographic Engineering or IEEE Transactions on Computers or CHES etc. would be better.



I have the following comments to improve the quality:
\begin{point}
Section II is given in a very brief manner. Details are needed for the previous studies. It does not serve state of the art. Mathematical background is not complete. I don't understand "As an example, performing a depth of four homomorphic multiplications with...". Why do we need this?  
\end{point}


\begin{reply}
Thank you for your valuable feedback on our paper. We appreciate your comments and suggestions, which have helped us to improve the quality of our work.

We agree with your comment that Section II needed more details. Therefore, we have revised and expanded Section II by providing a better explanation of the previous studies related to the Chinese remainder theorem (CRT) and number theoretic transform (NTT) for homomorphic encryption. 

First, we have added new subsections that discuss the need and motivation for using CRT and NTT in homomorphic encryption. We have also included a more detailed discussion of the previous studies related to these topics.

We apologize for the confusion caused by our statement about performing a depth of four homomorphic multiplications. We have revised the sentence to provide a better explanation. ``To implement homomorphic encryption in various applications, the depth-of homomorphic multiplication is one of the main factors that needs to be investigated, and increases proportionally with respect to the word-length of the coefficient. As an example, performing a depth of four homomorphic multiplications with an 80-bit security level requires a 180-bit ciphertext modulus and length-4096 polynomial in prior works~\cite{roy2019fpga}."
\end{reply}




\begin{point}
Section III has fundamental information about NTT. The connection with the proposed idea is not detailed. This section should be divided at least two parts. 
\end{point}



\begin{reply}
We agree with your comment about Section III in our previous manuscript and have revised it in the following ways.  

Specifically, we have divided Section III into two parts. The first part provides a more detailed explanation of the mathematical background for the low-complexity NTT-based polynomial multiplication algorithm, organized as a sub-section in Section II with detailed equations in the Supplementary Information. Section III now purely focuses on our proposed novel hardware design: parallel NTT-based polynomial multiplier without shuffling operations. We have provided a detailed explanation of our proposed design and its advantages compared to the prior works. We have also included a comprehensive analysis of the hardware complexity and performance of our proposed design.
\end{reply}


\begin{point}
Comparison is not fair. There are different studies on this. 
\end{point}

\begin{reply}
Thank you for bringing concern to our attention. Recognizing the inherent variation among different HE schemes, parameter settings, and hardware platforms in prior work, we have been very careful in our choice of baseline for comparison. We have selected~\cite{roy2019fpga} as the baseline, as it aligns closely with our FPGA device and parameter setting, providing the best-matched comparison for our proposed PaReNTT architecture design. In \secref{sec_ntt} and \secref{sec_crt}, we have discussed the application of our proposed optimization in different building blocks, followed by the theoretical complexity analysis compared with the prior work. We then evaluated these optimizations based on the experimental results and discussed them in \secref{result} in the revised manuscript.

It is important to point out that prior architectures were intended for edge devices. The emphasis in these architectures is on reduction of area and power. However, our proposed architecture is intended for the cloud. Thus, the emphasis is on reduction of latency and increase of sample speed. No prior architecture has addressed HE architectures for the cloud.
\end{reply}



\begin{point}
More details are needed for the experimental results.
\end{point}


\begin{reply}
Thank you for this insightful comment. We have added an additional sub-section in which we carry out a detailed analysis of our proposed residual coefficient computation unit and inverse mapping architecture to provide comprehensive experimental results to support our novel findings and optimizations in \secref{result}. Specifically, we have provided a comparison between our design for residual coefficient computation and the prior designs. Similarly, we also present a comparison and  analysis between our proposed implementation for inverse mapping of residual coefficients of polynomials and the conventional method. Pipelining and latency tradeoffs are investigated in the revised paper. 

We show that, compared to a prior design, the proposed
architecture reduces latency by a factor of 49.2, and the area-
time products (ATP) for the lookup table and DSP, ATP(LUT)
and ATP(DSP), respectively, by 89.2\% and 92.5\%. We show that for n=4096 and 180-bit coefficient, the proposed 2-parallel architecture requires 6.3 Watts of power while operating at 240 MHz.

\end{reply}

\begin{point}
Future works are much more attractive. Using CKKS gives better understanding.
\end{point}


\begin{reply}
Thank you for your valuable feedback. We appreciate your interest in the potential future developments of our work. While this work mainly concentrates on the CRT and NTT-based polynomial multiplier, we acknowledge the significance and the benefits of extending our design to the BFV and CKKS schemes. However, due to the space constraints in the current paper, a comprehensive and in-depth exploration of the optimization for these schemes will be considered in future work. Nevertheless, we believe integrating and customizing the proposed design into the BFV and CKKS schemes can significantly enhance the performance of those schemes. 
\end{reply}


\reviewersection

General comments:

The authors propose an efficient parallel residue arithmetic system for homomorphic encryption applications. The proposed approach has lower latencies since they avoid permutation of NTT outputs before inputting it to the iNTT block. Some modular simplifications helpful towards hardware implementation are considered. The area-block-processing product is maximized in the due course. The paper has the architectural details explained well. However, there are some specific comments that I have, useful for improving the paper further. 



\begin{point}
While the architecture is optimized in terms of latencies and area, there is also another component, which is the active and leakage power considerations. These could be a major issue when embedded to IoT devices and other edge applications where privacy is sought at the edge level. I did not notice any power optimization in the design. The authors must propose balanced architectures mindful of speed, power, area and leakage (SAPL) considerations. I know there are trade-offs. However, these design trade-offs are useful for designers to understand the choices made. These must be reflected in the architectural explorations and the results section. 
\end{point}


\begin{reply}
Thank you for your insightful comment. We appreciate your emphasis on the importance of SAPL considerations in hardware design. 

We report the power consumption of the proposed architecture. Specifically, we show that for $n=4096$ and 180-bit coefficient, the proposed 2-parallel architecture requires 6.3 Watts of power while operating at 240 MHz, with 6 moduli. With 4 moduli, the power consumption is 6.6 Watts. The CRT preprocessing part requires less complexity because of the novel decomposition approach, as compared with the 4-moduli architecture. 

The primary focus from previous hardware optimizations for HE schemes has prioritized low-area consumption, making them ideally suited for IoT and edge devices. However,  our work generally targets high-speed, low-latency, and high-throughput design, which is suitable for the cloud server. 

We have recognized the importance of a comprehensive analysis of timing, area, as well as power performance for the VLSI architecture design. Hence, the power consumption and a discussion on power performance have been included in \secref{result} of our revised manuscript. Unfortunately, direct power performance compared with the prior work~\cite{roy2019fpga} is not feasible due to the lack of power consumption data in their work. 


\end{reply}

\begin{point}
The decimation-in-time and decimation-in-frequency are standard well-known approaches. Are there other alternatives, optimized for e.g., the prime case? These details must also be worked out. 
\end{point}


\begin{reply}
We apologize for the confusion caused in Section III. In this work, instead of considering a low-complexity algorithm for NTT-based polynomial multiplication or the well-studied memory-based architecture, we present a novel real-time, feed-forward, high-throughput, and parallel NTT-based polynomial multiplication architecture design that does not require intermediate shuffling. We summarize our contribution to the proposed Parallel NTT-based polynomial multiplier without shuffling operations as follows. First, it eliminates the need for an intermediate shuffling circuit for a \textit{real-time} and feed-forward architecture, which can reduce the number of clock cycles required for computation. Second, the proposed architecture design is parameterized, making it easy to adjust to different input sizes and security levels. Third, the proposed design allows for an arbitrary level of pipelining, enabling high-speed operation. To address this comment, we have revised the discussion and clarified our contribution in Section III: ``In this section, we propose a novel real-time, feed-forward, high-throughput, and parallel NTT-based polynomial multiplication architecture design that does not require intermediate shuffling, as shown in \figref{polymult}. For a conventional implementation, an additional shuffling circuit is typically used for reordering output data before computing iNTT. However, such a shuffling circuit requires a large number of clock cycles and registers. In this proposed novel architecture, the two-parallel products are fed into a two-parallel iNTT architecture such that no intermediate buffer is needed. Thus, the outputs of the product are executed immediately by the iNTT. This is possible as we can select different folding sets for the NTT and iNTT. Moreover, the proposed architecture is generalized for any value of $n$, parameterized, and can achieve an arbitrary level of pipelining to achieve high-speed operation. ".


Additionally, since the degree of the polynomial used in HE schemes is required to be a power-of-two integer, the prime case is not considered. 

\end{reply}

\begin{point}
I would like to see a detailed analysis of optimized critical paths. These are mentioned briefly, for example in V. A, towards equation (20). It needs a thorough treatment. 
\end{point}


\begin{reply}
Thank you very much for your insightful comments. Pipelining tradeoffs are now investigated. The results for nonpipelined and pipelined pre-processing and inverse processing parts of the CRT are presented. To enhance the clarity and quality of our manuscript, all the pipelining cut sets have been highlighted in green in each corresponding building block. The discussion for these highlighted pipelining cut sets have been expanded.  
\end{reply}

\begin{point}
In Section V.C, it would be helpful to have normalized comparisons of the designs. These are particularly important when the frequency and other parameterics are not the same. Please mention the normalization approach and methodology to highlight how the proposed design is better over prior work. 
\end{point}


\begin{reply}
Thank you for your thoughtful feedback. To enhance the comparability and interpretability of our results, we have made the following adjustments in the revised manuscript. 

1) Our design has been reconfigured to align with the same parameter setting used in the prior work cited as~\cite{roy2019fpga}. The parameters are defined based on the 180-bit word-length of ciphertext modulus, consisting of six 30-bit co-primes, and the degree of the polynomial set at 4096.

2) To enable a fair comparison between our proposed design and prior work, we have normalized performance metrics. Specifically, we have chosen to compare latency in terms of $\mu$s to evaluate the timing performance.

3) For a comprehensive comparison of area performance, including LUTs and DSPs consumption, and timing performance, we have considered the area-timing product (ATP) for both LUTs and DSPs. The achieved reduction in ATP is presented as a percentage, highlighting the efficiency of our proposed design.

We have included a detailed discussion on these adjustments and the results, as referenced at \secref{result}.D.
\end{reply}


\begin{point}
The writing and organization could be improved. The abstract is too long. It could be significantly pruned. The Introduction is too long. Post introduction, a section could be introduced to describe homomorphic encryption at the system level before delving into the architectural details. 
\end{point}


\begin{reply}
We appreciate your constructive feedback and suggestions on the structure and length of our paper. In our revised manuscript, we have carefully revised and condensed the abstract and introduction sections, focusing on presenting the most critical information concisely. Additionally, to discuss homomorphic encryption at a system level, we have restructured the background section, which now begins with an overview of homomorphic encryption (HE), and then delves into the motivation behind and the contributions of our proposed designs in the context of HE.
\end{reply}

\begin{point}
Figure 1 is not very illustrative. How do you get ai(x)s? These details must be made very clear in the caption itself. Captions must be self-descriptive. They are too terse throughout the paper. 
\end{point}


\begin{reply}
Thank you for your valuable feedback. To improve the clarity of Figure 1, we have moved Figure 1 to Section IV and provided a detailed, step-by-step, mathematical explanation of how each variable/intermediate result is derived. This explanation is provided in the corresponding sub-sections.
\end{reply}

\begin{point}
Barrett units etc. must be motivated well for the general readership of the journal since these are specifics to the VLSI design community. 
\end{point}


\begin{reply}
Thank you for your comment. We have now motivated Barrett reduction and provided detailed explanation of how it is used.
\end{reply}

\begin{point}
Algorithm 1 has no comments and it is just a list of equations. I think it must be explained well. 
\end{point}


\begin{reply}
Thank you for your comment. We have moved the description of the low-complexity NTT/iNTT to the Supplementary Information (due to lack of space) and have included example flow graphs for $n=8$ in the main paper. We have also cited a tutorial preprint on this topic that we wrote~\cite{chiu2023nttbased}. This tutorial provides detailed derivations of three forms of NTT/iNTT for polynomial modular multiplication. 
\end{reply}



\newpage
